Uncertainty-Aware Learning for Improvements in Image Quality of the Canada-France-Hawaii Telescope

We leverage state-of-the-art machine learning methods and a decade's worth of archival data from CFHT to predict observatory image quality (IQ) from environmental conditions and observatory operating parameters. Specifically, we develop accurate and interpretable models of the complex dependence between data features and observed IQ for CFHT's wide-field camera, MegaCam. Our contributions are several-fold. First, we collect, collate and reprocess several disparate data sets gathered by CFHT scientists. Second, we predict probability distribution functions (PDFs) of IQ and achieve a mean absolute error of $\sim0.07''$ for the predicted medians. Third, we explore the data-driven actuation of the 12 dome "vents" installed in 2013-14 to accelerate the flushing of hot air from the dome. We leverage epistemic and aleatoric uncertainties in conjunction with probabilistic generative modeling to identify candidate vent adjustments that are in-distribution (ID); for the optimal configuration for each ID sample, we predict the reduction in required observing time to achieve a fixed SNR. On average, the reduction is $\sim12\%$. Finally, we rank input features by their Shapley values to identify the most predictive variables for each observation. Our long-term goal is to construct reliable and real-time models that can forecast optimal observatory operating parameters to optimize IQ. We can then feed such forecasts into scheduling protocols and predictive maintenance routines. We anticipate that such approaches will become standard in automating observatory operations and maintenance by the time CFHT's successor, the Maunakea Spectroscopic Explorer, is installed in the next decade.

==> app_all_together.tex <==
\section{Algorithm for probabilistic MPIQ prediction}
\label{sec:DL_putting_it_all_together}

\begin{algorithm}
\caption{Probabilistic MPIQ Prediction}
\label{algo:cont_norm}
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
%\renewcommand{\algorithmicinitialize}{\textbf{Initialize:}}
\REQUIRE matrices consisting of environmental and dome measurements for the labelled and unlabelled subsets ($\boldsymbol{\mathrm{X_{L}}} = \{x_{n}^{(1:d)}\}^{N_L}_{n=1}$ and $\boldsymbol{\mathrm{X_{U}}} = \{x_{n}^{(1:d)}\}^{N_U}_{n=1}$, respectively, where $N_L$ and $N_U$ are the number of samples in the labelled and the unlabelled subsets, and $d$ is the number of covariates/features), and MPIQ measurements for the labelled subset ($y_L = \{y_{n}\}^{N_L}_{n=1}$).
\ENSURE (i) predicted probability densities for both the labelled and the unlabelled datasets: $y_{L}\vert_\mathrm{pred} =\{y_{n}\vert_\mathrm{pred}^{(1),(2)}\}^{N_L}_{n=1}$ and $y_{U}\vert_\mathrm{pred} =\{y_{n}\vert_\mathrm{pred}^{(1),(2)}\}^{N_U}_{n=1}$. Each predicted PDF is characterized by a mean and a standard deviation. \\
(ii) feature importance matrices for both labelled and unlabelled subsets: $\boldsymbol{\mathrm{F_{L}}} = \{f_{n}^{(1:d)}\}^{N_L}_{n=1}$ and $\boldsymbol{\mathrm{F_{U}}} = \{f_{n}^{(1:d)}\}^{N_U}_{n=1}$.
\FOR{iteration $i_\mathrm{test}$ in range [1, 10]}
\STATE Divide $\boldsymbol{\mathrm{X_{L}}}$ into two subsets,a training subset $\boldsymbol{\mathrm{X_{L(train)}}}\vert_{i_\mathrm{test}}$, and a testing subset $\boldsymbol{\mathrm{X_{L(test)}}}\vert_{i_\mathrm{test}}$,in a $9:1$ ratio (i.e., 90\% training and 10\% testing); do this in a stratified cross validated manner (\S\ref{sec:DL_putting_it_all_together}).
\FOR{iteration $i_\mathrm{val}$ in range [1, 5]}
\STATE Sub-divide the training set into training and validation sets in a $4:1$ ratio; that is, $\boldsymbol{\mathrm{X_{L(train)}}}$ $\rightarrow$ $\boldsymbol{\mathrm{X_{L(train2)}}}\vert_{i_\mathrm{val}}$ and $\boldsymbol{\mathrm{X_{L(val)}}}\vert_{i_\mathrm{val}}$.
\STATE Combine $\boldsymbol{\mathrm{X_{L(train2)}}}\vert_{i_\mathrm{val}}$ with the unlabelled subset $\boldsymbol{\mathrm{X_{U}}}$, and train \textbf{INSERT MODEL NAME} on this collated dataset using the SaaS algorithm \textbf{cite SaaS algo here}. Obtain $y_{L(\mathrm{val})}\vert_\mathrm{pred, i_\mathrm{val}}$ by predicting on the validation set.
\ENDFOR
\STATE Use the collated predictions on all 10 validation sets to tune the hyperparameters of \textbf{insert model name} (\S\ref{sec:DL_putting_it_all_together}). Call this tuned model \textbf{insert model name}$_\mathrm{tuned}$.
\FOR{iteration $i_\mathrm{val}$ in range [1, 5]}
\STATE Using \textbf{insert model name}$_\mathrm{tuned}$, run $2,500$ iterations with Concrete Dropout (\S\ref{sec:DL_errors}) during inference, obtaining mixture model $\mu$ and $\sigma$ for samples in $\boldsymbol{\mathrm{X_{L(val)}}}\vert_\mathrm{i_\mathrm{val}}$.
\STATE Combine the $2,500$ $\mu$'s and $2,500$ $\sigma$'s for each sample using Equation \textbf{insert equation number} to obtain six values: $50^{th},$ $2.5^{th},$ and $97.5^{th}$ percentile confidence intervals for the mean $\mu$, lower prediction level $\mu - 1.96\sigma$, and upper prediction level $\mu + 1.96\sigma$.
\ENDFOR
\STATE Using \textbf{insert model name}$_\mathrm{tuned}$, make predictions on $\boldsymbol{\mathrm{X_{L(test)}}}\vert_{i_\mathrm{test}}$, and obtain six values per sample like above.
\STATE Obtain corresponding $2500$ feature importances during inference, and combine them using Equation (). Call the combined matrix $\boldsymbol{\mathrm{F_{L}}}\vert_{\mathrm{i_{test}}}$.
\STATE Use the collated predictions $y_{L}\vert_\mathrm{pred, al+epis, train}$ to calibrate the predictions on the test set, $y_{L}\vert_\mathrm{pred, al+epis, i_{test}}$, with Equation (). Call these $y_{L}\vert_\mathrm{pred, al+epis, cal, i_{test}}$.
\ENDFOR
\STATE Collate all $y_{L}\vert_\mathrm{pred, al+epis, cal, i_{test}}$ to obtain $y_{L}\vert_\mathrm{pred, al+epis, cal}$, and rename it $y_{L}\vert_\mathrm{pred}$.
\STATE Collate all $\boldsymbol{\mathrm{F_{L}}}\vert_{\mathrm{i_{test}}}$ and to obtain $\boldsymbol{\mathrm{F_{L}}}$.
\end{algorithmic} 
\end{algorithm}


==> app_ood_explanation.tex <==
\iffalse

\section{Out of Distribution}
\label{sec:ood}

\iffalse
\begin{figure*}
\centering
\begin{subfigure}{0.98\textwidth}
    \centering
    \includegraphics[width=0.98\linewidth]{figures/oodplot_0_20201011-042027.pdf}
    \caption{IQ$_{\textrm{Megacam}}$ x IQ$_{\textrm{MKAM}}$ after dome vent installation. IQ as a function of Wind Direction minus Dome pointing prior to dome vents.}
    \label{fig:my_label}
\end{subfigure}
\hfill
\begin{subfigure}{0.98\textwidth}
    \centering
    \includegraphics[width=0.98\linewidth]{figures/oodplot_1_20201011-042027.pdf}
    \caption{IQ$_{\textrm{Megacam}}$ x IQ$_{\textrm{MKAM}}$ after dome vent installation. IQ as a function of Wind Direction minus Dome pointing after dome vents.}
    \label{fig:my_label}
\end{subfigure}
\hfill
\begin{subfigure}{0.98\textwidth}
    \centering
    \includegraphics[width=0.98\linewidth]{figures/oodplot_8_20201011-042027.pdf}
    \caption{IQ$_{\textrm{Megacam}}$ x IQ$_{\textrm{MKAM}}$ after dome vent installation. IQ as a function of Wind Direction minus Dome pointing when dome vents are OPEN or CLOSED.}
    \label{fig:my_label}
\end{subfigure}
\end{figure*}
\fi

\begin{figure*}
    \centering
    \includegraphics[width=0.99\textwidth]{figures/oodplot_large_20201011-141451.pdf}
    \caption{Caption}
    \label{fig:ood}
\end{figure*}

Here, we analyze and visualize the impact that variable feature importance have on a model's predictions of the true mean and uncertainties. 

Assume that we have three categorical features $x_1$, $x_2$, and $x_3$ with 9 values each, for a total of 729 possible feature combinations.The target depends on the features as:
\begin{align}\label{eq:ood_distribution}
    y = \mathcal{N}\left(\mu=\mathcal{U}(x_1, x_2) + \lambda x_3, \sigma^2=\mathcal{C}(x_1, x_2)\right),
\end{align}
The output is normally distributed with a mean that depends on the first two features in a fixed way, and on the third feature in a variable fashion determined by the value of the modulating factor $\lambda$. A trivial value of $\lambda$ implies $x_3$ is a redundant feature with no predictive power, whereas an infinitely high (in magnitude) value signifies that $x_1$ and $x_2$ are relatively unimportant. $\sigma^2$ is the input aleatoric (or data) uncertainty, is dependent only on $x_1$ and $x_2$, and takes only two values -- 0.01 and 0.05 -- that are distributed as shown in the bottom-right square in Figure \ref{fig:ood}.

We consider four different cases with increasing values of the modulating factor $\lambda = 0, 1, 7, 255$. For each of these cases, the training set contains only 25 of the possible 81 configurations of $x_1$ and $x_2$, to simulate a scenario where we have access to only a subset of the entire parameter space. We place no such restriction on $x_3$, which is allowed to take all values from 0 to 8. The training set has 100 draws for each of the 225 ($25 \times 9$) points in the underlying 3-D parameter space (Equation \ref{eq:ood_distribution}), for a total of 22,500 samples. The test set consists of 729 samples -- a single draw per possible point in the parameter space. We use a  As can be seen from Figure \ref{fig:ood}, the impact of missing samples in the training set becomes less and less important as the underlying features $x_1$ and $x_2$ themselves becomes relatively less important in predicting the output $y$. 

\fi

\iffalse
Machine learning has been widely applied to a range of tasks. However, in certain high-risk applications, such as autonomous driving, medical diagnostics, and financial forecasting, a mistake can lead to either a fatal outcome or large financial loss. In these applications, it is important to detect when the system makes a mistake and take safer actions. Furthermore, it is also desirable to collect these “failure scenarios”, label them, and teach the system to make the correct prediction through active learning.
Predictive uncertainty estimation can be used for detecting errors . Ideally, the model indicates a high level of uncertainty in situations where it is likely to make a mistake. That allows us to detect errors and take safer actions. Crucially, the choice of action can depend on why the model is uncertain. There are two main sources of uncertainty: data uncertainty (also known as aleatoric uncertainty) and knowledge uncertainty (also known as epistemic uncertainty). If our goal is to detect errors, it is not necessary to separate these two uncertainties. However, if our goal is active learning, then we would like to detect novel inputs, and knowledge uncertainty can be used for that.
Data uncertainty arises due to the inherent complexity of the data, such as additive noise or overlapping classes. In these cases, the model knows that the input has attributes of multiple classes or that the target is noisy. Importantly, data uncertainty cannot be reduced by collecting more training data.
Knowledge uncertainty arises when the model is given an input from a region that is either sparsely covered by the training data or far from the training data. In these cases, the model knows very little about this region and is likely to make a mistake. Unlike data uncertainty, knowledge uncertainty can be reduced by collecting more training data from a poorly understood region.
\fi

==> app_sensorList.tex <==
\iffalse
\section{List of MegaCam sensor data}
\label{app:megaCamData}

\begin{table}
\begin{tabular}{|c|c|c|c|}\hline\hline%
Sensor & Units & Range & Description \\\hline\hline
\multicolumn{4}{l}{Environmental sensors} \\ \hline
Temp_1 & \degree C & XX & Temp.~ at XXX\\
Wind_1 & KPH & XX & Wind speed at\\
WindDir_1 & & & \\
WindDir_2 & & & \\
Pressure & & & \\\hline
\multicolumn{4}{l}{Observatory operating parameters} \\ \hline
Vents & & & \\
telAz & & &\\
telAl & & & \\
domeAz & & & \\
domeAl & & & \\
IQ & & & \\
skyBkgd & & & \\\hline
\multicolumn{4}{l}{Other instruments} \\ \hline
MKAM IQ & & & \\
MKAM_Az & & & \\
MKAM_Al & & & \\
\end{tabular}
\caption{Data fields in MegaCam dataset.}
\label{table:megaCamData}
\end{table}

this somewhat a rough all data table structure:
epoch, environmental (outside temperature, wind speed, wind direction, barometric pressure, etc.), CFHT facility ([instrument],[inside temperatures],vents[open or closed],telescope pointing, dome position or config, science data [iq, sky-background, etc.]), MKAM data (telescope pointing, seeing, mass[mass seeing profiles])
and this is what we're looking to populate to drive the analysis with:
epoch, MKAM seeing, MP IQ, WC IQ, ESP IQ, SIT IQ, SPI IQ,
\fi

==> data_availability.tex <==
\section{Data Availability}\label{sec:data_availability}
The data underlying this article are available in Zenodo, at \url{https://dx.doi.org/10.5281/zenodo.5295743}.

==> data_imputation.tex <==
\subsection{Data Imputation}\label{sec:DL_imputation}
Since neural networks can not automatically handle samples with different numbers of missing values, this calls for feature imputation. In this work, we accomplish this in the \emph{pre-training} phase--we train the complete subset $D_{comp}$ in a \emph{self-supervised} manner, using a Sliced Wasserstein Autoencoder (SWAE, Figure (), \cite{sliced_wasserstein_autoencoder_swae})\footnote{The SWAE is a simpler version of the Wasserstein Autoencoder \citep{wasserstein_autoencoder}, and has been shown to perform almost as well but with a much simpler architecture (\textbf{check this})}. Self-supervised learning is a regime of deep learning that enables us to reconstruct the input data without the use of labels. Here, we do not care about precise prediction of MPIQ, but are interested in learning a good intermediate representation with the expectation that this can approximate well the `true', underlying generative distribution. As can be seen from Figure (), of the total () samples/observations in our corpus, () (or $\approx x \%$) contain no missing values. We use these () samples to train our SWAE using the mean absolute error (MAE) loss function. Once training converges (based on cross-validation results), we use the method proposed by \cite{autoencoder_imputation} to impute the missing values for the remaining () out-of-sample observations. In brief, this process is as follows: (a) For the out out-of-sample observations, use a relatively simple imputing scheme to fill in the missing values. Here we use k-NN imputation () from \textsc{pandas}, which fills missing features with mean values of those features cmoputed from the $k$ nearest training samples (we used $\text{k} = 5$). (b) Use the auto-encoder network (SWAE) trained on the complete sub-set, for inference on the incomplete sub-set. Iteratively update $\hat{x}_{J}$ using $\hat{x}_{J}^{t+1}=\hat{x}_{J}^{t}+h\left[f\left(\hat{x}^{t}\right)-\hat{x}^{t}\right]_{J}$, where $f$ is the trained SWAE, $h$ is a step size and $\hat{x}^{t}=\left(\hat{x}_{J}^{t}, x_{J^{\prime}}\right) \in \mathbb{R}^{d}$ denotes a complete point where the observed components are fixed at the observed values and the missing ones are replaced by the current estimate. We use h=0.001, and in Figure () plot $\hat{x}_{J}^{t+1} - \hat{x}_{J}^{t}$ averaged over all samples in the incomplete set. We stop updating at time step (), when gains start diminishing.%\yst{Then you need to explain what is self-supervised. If most of the data does not require inputating, and the additional self-supervised learning does not help much, this part should be simplified with simple supervised learning}
\yst{I am not sure I fully follow the connection between the (a) and (b). My naive understanding is that here you train an auto-encoder, and each time you find k-nearest neighbour in the latent space, and use the mean to update the inputted values. In this case, I am not sure I understand $\hat{x}_{J}^{t}+h\left[f\left(\hat{x}^{t}\right)-\hat{x}^{t}\right]_{J}$. For me it seems like the two terms are not the tensor of same dimension. Maybe elaborate?}

==> eda.tex <==
\subsection{Exploratory Data Analysis}\label{sec:eda}

\begin{figure*}
\begin{subfigure}{0.33\textwidth}
\centering
    \includegraphics[width=0.98\linewidth]{2005-2020_Histograms_OPEN_CLOSED_MPMK.png}
    \caption{IQ$_{\textrm{Megacam}}$ x IQ$_{\textrm{MKAM}}$ prior to dome vent installation. Median Megacam IQ compared to Mediam MKAM Seeing prior to installation of dome vents.}
    \label{fig:my_label}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
\centering
    \includegraphics[width=0.98\linewidth]{2005-2020_Histograms_OPEN_CLOSED_MPMK_a.png}
    \caption{IQ$_{\textrm{Megacam}}$ x IQ$_{\textrm{MKAM}}$ after dome vent installation. Median Megacam IQ compared to Median MKAM Seeing after installation of dome vents. (This also demonstrates data cadence issues as MKAM has failed often since the dome vents were installed.)}
    \label{fig:my_label}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
\centering
    \includegraphics[width=0.98\linewidth]{2005-2020_Histograms_OPEN_CLOSED.png}
    \caption{IQ$_{\textrm{Megacam}}$ x IQ$_{\textrm{MKAM}}$ after dome vent installation. Median Megacam IQ compared to Mediam MKAM Seeing when dome vents are OPEN or CLOSED.}
    \label{fig:my_label}
\end{subfigure}
\caption{Put caption here}
\label{fig:hists}
\end{figure*}


\begin{figure*}
\begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=0.98\linewidth]{2005-2020_WindDomeAzi_MPIQ_0.png}
    \caption{IQ$_{\textrm{Megacam}}$ x IQ$_{\textrm{MKAM}}$ after dome vent installation. IQ as a function of Wind Direction minus Dome pointing prior to dome vents.}
    \label{fig:my_label}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=0.98\linewidth]{2005-2020_WindDomeAzi_MPIQ_0_a.png}
    \caption{IQ$_{\textrm{Megacam}}$ x IQ$_{\textrm{MKAM}}$ after dome vent installation. IQ as a function of Wind Direction minus Dome pointing after dome vents.}
    \label{fig:my_label}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=0.98\linewidth]{2005-2020_WindDomeAzi_MPIQ_0_b.png}
    \caption{IQ$_{\textrm{Megacam}}$ x IQ$_{\textrm{MKAM}}$ after dome vent installation. IQ as a function of Wind Direction minus Dome pointing when dome vents are OPEN or CLOSED.}
    \label{fig:my_label}
\end{subfigure}


\begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=0.98\linewidth]{2005-2020_TEAMIRCI_TEAMIRCO_MPIQ_0.png}
    \caption{before dome vent installation temperature imbalances at the mirror}
    \label{fig:my_label}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=0.98\linewidth]{2005-2020_TEAMIRCI_TEAMIRCO_MPIQ_0_a.png}
    \caption{after dome vent installation temperature imbalances at the mirror persist}
    \label{fig:my_label}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=0.98\linewidth]{2005-2020_TEAPMSPS_TEAPMCLW_MPIQ_0.png}
    \caption{before dome vent installation temperature imbalances at the mirror example 2}
    \label{fig:my_label}
\end{subfigure}


\begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=0.98\linewidth]{2005-2020_TEAPMSPS_TEAPMCLW_MPIQ_0_a.png}
    \caption{after dome vent installation temperature imbalances at the mirror persist example 2}
    \label{fig:my_label}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=0.98\linewidth]{2005-2020_TEMPERAT_TEATOPWS_MPIQ_0.png}
    \caption{before dome vent installation temperature imbalances at the top of the dome}
    \label{fig:my_label}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=0.98\linewidth]{2005-2020_TEMPERAT_TEATOPWS_MPIQ_0_a.png}
    \caption{after dome vent installation temperature imbalances at the top of the dome are lessened}
    \label{fig:my_label}
\end{subfigure}
\caption{Put caption here}
\label{fig:eda}
\end{figure*}


==> instruments.tex <==
\begin{itemize}
\item \emph{Wide-field InfraRed Camera (WIRCam):} WIRCam  is the near infrared mosaic imager mounted at the prime focus of the 3.6m CFHT telescope. It saw first light in November 2006 and has been offered for science in all observing semesters since February 2006. 
WIRCam has a field of view of 20 sq.min. The WIRCam focal plane is made of a mosaic of four HAWAII2-RG detectors, each containing 2048 x 2048 pixels, with a sampling of 0.3 arc second per pixel. WIRCam is fitted with an image stabilization unit (ISU) using on-chip guiding. During an exposure, the image stabilization signal is obtained by repeatedly reading out a small, 14x14 pixel region centered on a bright star on each of the four detectors, while the integration continues uninterrupted for the rest of the pixels. The nominal near-infrared seeing of 0.8 arc.sec measured at the CFHT site on Mauna Kea is well sampled by the 0.3 arc.sec pixel scale of WIRCam, making it adequate for most science programs. However, occasionally the seeing has been observed to improve to 0.5 arc.sec or better, under which the PSF becomes undersampled. In order to facilitate science programs which can benefit from such exceptional seeing conditions, WIRCam can use its image stabilization unit to micro-step the image with 0.15 arc.sec sampling. 
\item \emph{Mauna Kea atmospheric monitor (MKAM)} MKAM is a collaborative project between IFA (Institute for Astronomy, University of Hawaii), CFHT and W.M. Keck. The goal of which is to install a seeing monitor on the CFHT site for use by all the observatories on the summit.  Provides a measure of the Fried parameter (r0) at a wavelength of 0.5 microns with a goal of an precision of better than $5\%$ at the observed zenith angle and azimuth and an estimate of r0 corrected to the zenith. The r0 value should be corrected for the finite exposure time of the instrument. Goal of an accuracy of $5\%$ in r0 and the measurements will be from at least six meters above grade.
Fried's parameter r0 quantitatively expresses the image degradation due to atmospheric turbulence.  r0 represents the diameter of the coherent cells in the incident wave at the telescope pupil.
\url{http://articles.adsabs.harvard.edu//full/1981SoPh...69..223R/0000227.000.html}
the MASS profiler is an instrument in addition to the DIMM in MKAM.
MASS Turbulence Profiler. MASS is an instrument to measure the vertical distribution of turbulence in terrestrial atmosphere by analysing the scintillation (twinkling) of bright stars. When stellar light passes through a turbulent layer and propagates down, its intensity fluctuates.
another reference to cfht/rene/r0 from keck...
https://www2.keck.hawaii.edu/optics/kpao/files/KAON/KAON303.pdf
in particular item 2.
and from Tokovonin 
https://iopscience.iop.org/article/10.1086/428930
\end{itemize}

\iffalse
\emph{Echelle SpectroPolarimetric Device (ESPaDOnS)}: ESPaDOnS is a bench-mounted high-resolution echelle spectrograph and spectropolarimeter which was designed to obtain a complete optical spectrum (from 370 to 1,050 nm) in a single exposure with a resolving power of about 68,000 (in spectropolarimetric and 'object+sky' spectroscopic mode) and up to 81,000 (in 'object only' spectroscopic mode). ESPaDOnS was commissioned and fully operational by February 2005. 

\emph{Spectromètre Imageur à Transformée de Fourier pour l'Etude en Long et en Large de raies d'Emission(SITELLE)} SITELLE is the optical imaging Fourier transform spectrometer (IFTS) at CFHT that saw first light in July 2015. It provides integral field unit (IFU) spectroscopic capabilities in the visible spectrum (350 to 900 nm) over an $11' \times 11'$ field of view, with a variable spectral resolution, depending on the requirement of the observer, from R=2 to R>104 (for low to high spectroscopic studies). The SITELLE focal plane is made of 2 cameras, each of them a four output 2048 x 2048 pixels, low noise, CCD231-42 e2v chip that allows attaining 5e noise in 1 second read time and 3.5 electron in 2 seconds. The nominal optical seeing of 0.8 arcsec measured at the CFHT site on Mauna Kea in the R band is well sampled by the 0.32 arc.sec pixel scale of SITELLE, making it adequate for most science programs. SITELLE will therefore provide about 1 million independent spectra at once. 

\emph{SPectropolarimètre InfraROUge (SPIRou)} Near-infrared spectropolarimeter with high radial-velocity precision  SPIRou is fiber-fed from the Cassegrain focus of the CFHT. The SPIRou Cassegain unit includes a polarimeter to change the polarization of the incident light and derive linear or circular polarization states of the observed target. The SPIRou spectrograph is embedded in a cryogenic vessel cooled down to a temperature of 80 K and stabilized at a precision below 2 mK. The spectrograph provides YJHK spectra from 0.95 to 2.35 microns in a single shot, at a spectral resolution of ~75,000. SPIRou will use an Hawaii 4RG detector, which is currently in the making at Teledyne Scientific and Imaging. It will have 4kx4k 15-micron pixels that will be read continuously in order to leave the cryostat temperature undisturbed. Since it is to be delivered after the lab tests in France, the SPIRou team is using an Hawaii H2RG 2kx2k detector with 18 microns pixels for alignments and performance tests. This detector covers a large fraction of the spectral range and gets most of the spectral resolution. \fi



==> list_of_figures.tex <==

\section{List of Figures}\label{sec:list_of_figures}
\begin{itemize}
    \item Schematic of Telescope, with vents and angles highlighted: \textbf{half a page?}
    \item \textbf{1 full page}, final network:
    \begin{itemize}
        \item Sliced Wasserstein AutoEncoder (SWAE) + Imputation block
        \item Tabnet block (modify from \cite{tabnet}
        \item Speed as a Supervisor (SaaS) block (modify from \cite{saas2})
        \item Mixture Density Network (MDN)
    \end{itemize}
    \item \textbf{1x1}: Show convergence of imputation (\S\ref{sec:DL_imputation})
    \item Exploratory Data Analysis (EDA) plots from Billy's work:
    \begin{itemize}
        \item divide features into groups. temperature, temperature difference, (insert more here). for each group, identify the top two feature with strongest correlations with mpiq, and show two figures with two plots each--mpiq $\ge$ mkamiq, with vents open and closed, repeat for mpiq $<$ mkamiq. for each group, a total of 4 subplots (2 per feature), arranged in \textbf{2x2} fashion. for a total of \textbf{k} such plots, for k groups.
        \item anything else?
    \end{itemize}
    \item EDA plots from Racine's work. still need to finalize.
    \item Probability Calibration (\S\ref{sec:DL_probability_calibration}), Errors (\S\ref{sec:DL_errors}).
    \begin{itemize}
        \item \textbf{1x3}, or \textbf{1x2 + 1x1}. point predictions, aleatoric errors + epistemic errors, aleatoric+epistemic WITH probability calibration. in each plot, jot down all the metrics from \S\ref{sec:DL_metrics}.
    \end{itemize}
    \item Benefit of MDN (\S\ref{sec:DL_MDN}):
    \begin{itemize}
        \item \textbf{2x2} plot: for gaussian:for the two cases of with and without mdn, joint plot of median predictions vs ground truth. repeat the same for beta.
        \item \textbf{1x1} plot: histogram of mpiq fitted with gaussian and fitted with beta, to demonstrate the superiority of the latter.
    \end{itemize}
    \item Feature Importance
    \begin{itemize}
        \item \textbf{1x1} summary plot with positive and negative correlations. \textbf{need to write code to combine the two}
        \item \textbf{1x2} Evolution of Feature Importance with time, with clustering. \textbf{need to write code for this}.
    \end{itemize}
    \item SSL (\S\ref{sec:DL_SSL}): \textbf{1x2} pred v/s true (calibrated). for both, jot down all metrics. SSL should show improved results.
    \item \textbf{1x2}: Compare performance to NGBoost + Shap
\end{itemize}


==> list_of_tables.tex <==
\section{List of Tables}\label{sec:list_of_tables}
\begin{itemize}
    \item Example dataset. \textbf{One row, both columns}. Use caption to explain the features in some detail.
    \item Benefit of MDN: \textbf{1x1, 2 columns, 7 rows}: table of metrics, comparing results with and without mixture model.
\end{itemize}


==> mdn.tex <==
\subsubsection{Mixture Density Network}\label{sec:DL_MDN}

Mixture density networks (MDNs) are composed of a neural network and a mixture model\footnote{In their initial form~\cite{bishop_mdn}, MDNs used a Gaussian mixture model (GMM); they can  easily be generalized to other distributions.}. We begin by recapping the concept of a mixture model--a model of probability distributions built up from a weighted sum of more simple distributions. More concretely, we consider a 

In a one-dimensional mixture model with $m$ components the overall probability density function (PDF) 
\[
p(x)=\sum_{j=0}^{m-1} \omega_{j} p_{j}(x)
\]
is weighted sum of $m$ PDFs $p_{j}(x)$ with non-negative weights $\Omega=\left\{\omega_{0}, \ldots, \omega_{m-1}\right\}$; where $\sum_{j=0}^{m-1} \omega_{j}=1$.

Typically these probability distributions will be parameterised by a series of parameters that reflect the shape and location of the distribution $\Theta=\left\{\theta_{0}, \ldots, \theta_{m-1}\right\} .$ The full parameterised model may therefore be written as
\[
p(x \mid \Omega, \Theta)=\sum_{j=0}^{m-1} \omega_{j} p_{j}\left(x \mid \theta_{j}\right)
\]
As an example, each $p_{j}$ could be a normal distribution parameterised by a mean $\mu_{j}$ and a variance $\sigma_{j}$. The mixture model would then have the following form,
\[
p(x \mid \Omega, \Theta)=\sum_{j=0}^{m-1} \frac{\omega_{j}}{\sqrt{2 \pi \sigma_{j}^{2}}} \exp \left(\frac{-1}{2 \sigma_{j}^{2}}\left(x-\mu_{j}\right)^{2}\right)
\]
In general, these mixture distributions are multi-modal, including those in the form of Eq
$(4),$ and can be fitted directly to some data $\mathbf{x}=\left(x_{0}, \ldots, x_{n-1}\right) .$ Assuming independence, the corresponding likelihood is calculated as
\[
l(\mathbf{x} \mid \Omega, \Theta)=\prod_{i=0}^{n-1}\left[\sum_{j=0}^{m-1} \omega_{j} p_{j}\left(x_{i} \mid \theta_{j}\right)\right]
\]
Fitting can then typically proceed using expectation-maximisation [20] \yst{Is this correct? For our case, there are no classes, the training should only be a maximum likelihood. Am I missing something here? Or do you mean classical GMM here. I would shorten this.}. For our purposes, we have an individual-based model $M,$ with some input $\alpha,$ that produces stochastic realisations $y \sim M(\alpha) .$ We therefore wish to derive a relationship between the input parameters $\alpha,$ and the mixture density weights $\omega_{j}(\alpha)$ and density parameterisations $\theta_{j}(\alpha) .$ This could potentially be done with a separate regression for each of the density parameters and weights, although this would fail to capture the corresponding relationships that would exist between each parameter and weight. We can therefore model these using a neural network, which is able to provide flexible fitting for arbitrarily complex relationships by the universal approximation theorem
$[22] .$ An MDN is therefore defined as a mixture model, where the mixture components are modelled using a neural network. Fig 1 provides an overview of the MDN construction. The inputs of the model $\alpha$ are initially fed into the MDN (three such inputs in the example diagram). These are then passed through a number of hidden layers in the neural network, which provide a compact representation of the relationship between the inputs and the unnormalised inputs into the mixture model. These distribution parameters are then passed through a normalisation layer; the weights of the mixture are transformed such that they sum to one and the shape parameters are transformed so that they are positive. These parameters are used to construct the mixture model, where one can draw samples or calculate statistics, such as mean and variance, for a given input. For multiple outputs the final layer can be copied with independent parameters for the number of outputs being considered \yst{Not sure I follow the last sentence here?}. Note that a number of aspects of the MDN need to be specified including the number of input parameters, the dimension of the output, the distributions used in the mixture density, and the number and size of the hidden layers.
The MDN can then be fit to the following objective loss function, which is equivalent to maximising the likelihood given in $\mathrm{Eq}(5)$
\[
f(\mathbf{x} \mid \Omega, \Theta)=-\sum_{i=0}^{n-1} \log \left(\sum_{j=0}^{m-1} \omega_{j} p_{j}\left(x_{i} \mid \theta_{j}\right)\right)
\]
Note that provided $p_{j}$ is differentiable with respect to $\theta_{j}$, this loss represents a differentiable function. Standard techniques based on stochastic gradient descent can then be applied in order to optimise the weights of the network with respect to this loss [23]

Mixture density networks (MDN) (Bishop, 1994) are a class of models obtained by combining a conventional neural network with a mixture density model.
We use a mixture of 20 normal distributions parameterized by a feedforward network. That is, the membership probabilities and per-component mean and standard deviation are given by the output of a feedforward network.


The standard normal--or Gaussian--distribution acts as the
foundation for countless modeling approaches in statistics
and machine learning. As opposed to a single Gaussian,
which is a very limited model, \emph{Gaussian mixture models} can represent or approximate almost any density
of interest while remaining intuitive and easy to handle. A Gaussian is characterized by two parameters--mean $\mu$ and standard deviation $\sigma$. We see from Figure () that our output label of interest, MPIQ, does not resemble a Gaussian

\begin{figure*}
   \centering
    \includegraphics[width=\textwidth]{Fig3.png}
    \caption{Optimizing the vent configuration can dramatically improve the image quality of the telescope. \textbf{(3a)} shows the nominal vent configurations, and \textbf{(3b)} the (predicted) optimal vent configuration that leads to the IQ improvements shown in \textbf{(3c)}. The red dashed lines in \textbf{(3c)} delineate the assumed improvements for the exposure time calculation.}
    \label{fig:actionable}
\end{figure*}

\iffalse
\begin{figure*}
    \centering
    \begin{subfigure}
    \includegraphics[width=.49\textwidth]{shap_heatmap_goodsmall.png}
    \caption{Caption}
    \label{fig:my_label}
    \end{subfigure}
\end{figure*}
\fi
\yst{I think here you also need to explain how you define aleatoric and epistemic uncertainties from the MDN output. E.g, sigma of the mean, and mean of the sigma.}


==> ml_baseline.tex <==
\subsection{Light GBM}\label{sec:ml}
(\sg{waiting on sebastien})

==> ml_vs_dl.tex <==
\subsection{Boosted Trees and Deep Neural Networks}\label{sec:ml_vs_dl}
%\Simon{although this section is very interesting per se, I believe it should probably be shortened quite a bit, summarizing the main advantages of a network w.r.t. to tree-based methods, especially in view of streaming data.}
%While DNNs allow extraction of significantly richer patterns between inputs and output(s), they have earned a reputation for being `black-boxes' -- it can be difficult to explain the series of steps a neural network takes to find the relationships between the input features and the output(s) of interest. This is where tree-based models shine -- they are designed to be agglomeration of `if-then-else' statements, thus making it considerably easier to inspect the relationships both between the input features and the outputs, as well as among the features themselves. They pay a price for increased interpretability with decreased ability for feature extraction\footnote{That is, a machine learning model can only work with the user-provided features, whereas a deep enough neural network, in theory, can construct arbitrary complex combinations of these features if such an exercise results in better prediction of the output variable(s) of interest.}, and often times are not the tools of choice for \emph{unstructured data} -- images, videos, text and audio \citep{tabnet}. 

%This hierarchy, however, is reversed in the case of \emph{structured}, tabular\footnote{Tabular data is considered `structured' because typically a human decides to put the features (columns) and observations (rows) in a certain order, whereas images, audio and languages have a naturally occurring order and do not need to be `structured' by the user.} data, where features are individually meaningful and lack strong multi-scale temporal or spatial structures; in this setting, gradient boosted decision trees (GBDT) \citep{gradient_boosted_decision_trees_gbdt, xgboost, catboost} perform reasonably well.
%preferred for their exmore often than not outperform standard deep models on tabular-style datasets \citep{tabnet}, where features are individually meaningful and lack strong multi-scale temporal or spatial structures; the state-of-the-art performance in problems with tabular heterogeneous data is often achieved by such as gradient boosted decision trees (GBDT) \citep{gradient_boosted_decision_trees_gbdt, xgboost, catboost}.
%This raises two questions: (i) \emph{why} does deep learning perform poorly on tabular data, and (ii) \emph{how} can we fix it? \seb{not exactly sure that DL can be said to perform poorly on tabular data anymore - as it is examplified here.} \yst{agreed. This is an unnecessary shot/comparison} The key to answering question (i) is to understand the ways in which tabular data are fundamentally different from unstructured data:


%Our dataset consists of heterogeneous, sparse, and categorical data.  The dataset is heterogeneous due to the wide variety of sensors (wind speed, temperature, telescope pointing) each recorded in specific  units.  The dataset is sparse due to lost data, sensor failures, and sensor replacement or re-positioning.  The dataset is categorical (rather than continuous) because sensor measurements are often binned, e.g., wind speed below $5$ knots, $5$-$10$ knots, etc.  These characteristics induce a discontinuous feature space.  Tree-based models such as decision trees~\citep{decision_trees}, random forests~\citep{randomforests}, and gradient boosted trees \citep{xgboost, lightgbm} are well-matched to these data characteristics. Tree-based models select and combine features greedily to whittle down the list of pertinent features to include only the most predictive ones. Tree-based models easily handle categorical features using, e.g., one-hot encoding. Further, feature sparsity and the presence of NULL values is easily accommodated by such models,  they simply do not include feature cells containing such values in their splits.  In this paper we implement an off-the-shelf Light GBM model to provide a performance baseline. To extract feature importance and interactions from this tree-based model, we use the SHAP package \citep{shap1,shap2}.%; we expound on this in \S\ref{sec:DL_feature_imp}. 

Tree-based models such as simple decision trees~\citep{decision_trees}, random forests~\citep{randomforests}, and gradient boosted trees \citep{gradient_boosted_decision_trees_gbdt} are well-matched to these data characteristics. Tree-based models select and combine features greedily to whittle down the list of pertinent features to include only the most predictive ones. Further, feature sparsity and missing data is naturally accommodated by tree models, they simply do not include feature cells containing such values in their splits.  In this paper we implement an off-the-shelf model gradient boosting tree model to provide a performance baseline. To extract feature importance and interactions from this tree-based model, we use the SHAP package \citep{shap1,shap2}.%; we expound on this in \S\ref{sec:DL_feature_imp}. 
%\tcr{(SCD: Sankalp, can you work back over the second half of the following paragraph and pass back to me -- starting from "we overcome several deficiencies")}

However tree-based models require the human process of feature engineering and have been shown \citep{bengio2010decision} to poorly generalize.
In contrast to tree-based models, deep neural networks (DNNs) are powerful feature pre-processors. Using back-propagation, they learn a fine-tuned hierarchical representation of data by mapping input features to the output label(s). This allows us to shift our focus from feature engineering to fine-tuning the architecture, designing better loss functions, and generally experimenting with the mechanics of our neural network. As we will show, our neural network with little to no feature engineering \seb{Are we really doing no feature engineering for the MDN?}  performs better than the alternative tree-based boosted model that uses extensive feature engineering. In reported comparison cases, DNNs yield improved performance with larger sized datasets \citep{airbnb}. 

% SF: an interesting case, but not clear to me how DNN is a no-brainer for online-learning, and why we should worry about it in the future for our project.

%Finally, it is more natural to use DNNs in an online-mode, with data points `streaming in' rather than arriving in batches. On the other hand, tree-based models need access to all the data to determine best split points, and hence need to be trained every time a new observation comes in. While we do not use a large dataset (we have $\sim 60,000$ samples), or streaming data, in preparation for our future work on real-time predictions we believe it important to consider neural network models from the start.

%Turning to neural networks, the ideal architecture would be one designed to handle the peculiarities of the tabular data discussed above.  However, for the most part, neural networks are designed for unstructured data. While, as mentioned in Section \ref{sec:relatedWork}, there has been some work done in applying neural networks to tabular data \citep{milli2019nowcasting_paramal},  there remains significant room for improvement.

%In this paper, we overcome several deficiencies of traditional neural networks when applied to tabular data by designing and utilizing a feed-forward mixture density network (MDN) as depicted in Figure \ref{fig:1-to-1_plus_mdn}. %\Simon{Motivation for the MDN should be introduced here. Since we are not using DIMM information, atmospheric seeing acts here as a noise source with complex, heteroschedastic properties that an MDN is good at addressing}
%The VAE is capable of handling missing observations in data, as well as identifying which samples in its training set contain errant values, and hence allows us to use the versions of our input data containing all samples, $\mathcal{D_{F_L,S_L}}$ and $\mathcal{D_{F_S,S_L}}$.
%On the other hand, atmospheric seeing acts as a noise source with complex, heteroschedastic properties that an MDN is good at addressing. We use \texttt{BatchNorm} layers \citep{batchnorm} after the input layer of the MDN so that all features are placed on the same scale and none of them unduly affects the gradients and weights during flow through the network. For accessing feature importance and interactions, we use the recently open-sourced \textsc{Python} package \texttt{pathexplain}\footnote{\url{https://github.com/suinleelab/path_explain}} \citep{explaining_explanations_hessians}. 

\iffalse
\tcb{(SCD: I suggest we deleted the rest of the following})

\tcb{++++++++DELETE REST OF SUBSECTION++++++++++}

Neural networks face extra challenges when being applied to structured data while tree-based models

The structured data sets we work with have a number of characteristics that are important to note.
\begin{itemize}
    \item {\bf Heterogenity:}  Feature come from disparate sources, each with their own units. In our case the features included, e.g., environmental sensor measurements, observatory telemetry, and measured instrumental image quality.
    \item {\bf Sparsity:} Unlike data from audio, video and language, there can be relatively little variation in the values of a column in a table. There are often NULL values where no data was collected, or was lost or corrupted in the collation process. \tcr{(SCD: Sankalp, I don't get the point about the ``relatively little variation'')}
    \item {\bf Categorical:}  Feature are often categorical indicating, e.g., that the wind speed is below $5$ knots, between $5$ and $10$ knots, between $10$ and $20$ knots, or above $20$ knots.  In contrast, image pixel values are typically integers between $0$ and $255$ which is better modeled as a continuous range.
    \item {\bf Correlation:}  A minority of the columns in a table are often responsible for the majority of the predictive power. This is unlike the case for images, for instance, where in spite of local spatial correlations between pixels, it is difficult to claim, e.g., that it is the top-left cluster of them that is most helpful in predicting whether an image contains a cat or a dog. \tcr{(SCD: Simon makes a good comment about images being low-entropy, do we keep this or remove?)}
    \Simon{Here again, I would not define input correlations as specific to tabular data. Natural images e.g. have relatively low entropy - and hence can usually be compressed efficiently - and this in turn implies correlations between pixels}
\end{itemize}

%These issues complicate analysis of tabular data with DNNs.
These differences from unstructured data lead to a sparse and discontinuous high-dimensional feature space, making it difficult to exploit for deep neural networks (DNNs). On the other hand, tree-based models -- decision trees \citep{decision_trees}, random forests \citep{randomforests}, and gradient boosted trees \citep{xgboost, lightgbm} -- naturally profit from this landscape. They are by design able to select and combine features via a greedy heuristic, and thus whittle down the list of pertinent features to just the most predictive ones. They are also able to easily handle categorical features using any number of encoding schemes, the most commonly used one being one-hot encoding. The sparsity of features and the presence of NULL values is not of concern to them either, since they simply do not include feature cells containing such values in their splits.

Given the great fit between tree-based models and tabular data, the obvious question arises -- why even consider neural networks?
\begin{itemize}
    \item DNNs are powerful feature pre-processors. Using back-propagation, they learn a fine-tuned hierarchical representation of data by mapping input features to the output label(s). This allows us to shift our focus from feature engineering to fine-tuning the architecture, designing better loss functions, and generally experimenting with the mechanics of our neural network. As we show in Figures (xxx) and (xxx), our neural network with little to no feature engineering performs better than the alternative tree-based boosted model that uses extensive feature engineering.
    \item There is empirical proof that DNNs result in improved performance with larger sized datasets \citep{airbnb}.
    %\item Deep learning allows us to train systems end-to-end, which unlocks the possibility of using unlabelled samples to better predict the labelled ones (\emph{semi-supervised learning}, \S\ref{sec:DL_SSL}).
    \item %\Simon{This is probably a crucial argument for DNNs, as our input data set is here bound to grow with time}
    It is easier to use DNNs in an online-mode, with data points `streaming in' rather than arriving in batches. This is because tree-based models need access to all the data to determine best split points, and hence need to be trained every time a new observation comes in. While this work does not use streaming data, in preparation for our future work on real-time predictions we believe it best to move to a neural network from the get-go.
    \item Finally, tree-based models have been known to generalize poorly (\sg{Sebastien: you suggested this; can you expand + put in a couple of citations please?}).
\end{itemize}
%\input{tabnet}
\fi
%Clearly, the ideal model for working with the kind of tabular data we have from CFHT would be a neural network that is designed to handle the peculiarities of tabular data listed above, and is also easily explainable. As mentioned in Section \ref{sec:relatedWork}, there has been some work done in this field \citep{milli2019nowcasting_paramal}, but there is significant room for improvement. 


%\tcr{(SCD: Sankalp, Should these next two paragraph go here?  The previous two paragraph, respectively, discussed the data + tree-based models, and the NNets.  The next paragraph talks about "deficiencies of tree-bsead models" but the previous paragraph discussed deficiencies / challengaeas of NNets, so the transition is unclear.  I feel the paragraph really is discussing how we surmount the challenges facing the application of NNets to categorical data.  Is this what you're after?  And, if it is, should it go here?  (Maybe, b/c we discussed challenges faced by NNets)}


% SF: commented to move further
%For these reasons, in this paper we design and utilize a feed-forward mixture density network (MDN) as depicted in Figure \ref{fig:1-to-1_plus_mdn}. An MDN is able to capture the complex, heteroschedastic properties of seeing (IQ), and easily able to output uncertainties. 

%\Simon{Motivation for the MDN should be introduced here. Since we are not using DIMM information, atmospheric seeing acts here as a noise source with complex, heteroschedastic properties that an MDN is good at addressing}
%The VAE is capable of handling missing observations in data, as well as identifying which samples in its training set contain errant values, and hence allows us to use the versions of our input data containing all samples, $\mathcal{D_{F_L,S_L}}$ and $\mathcal{D_{F_S,S_L}}$.
%On the other hand, atmospheric seeing acts as a noise source with complex, heteroschedastic properties that an MDN is good at addressing.


% SF: commented to move further
%We use \texttt{BatchNorm} layers \citep{batchnorm} after the input layer of the MDN so that all features are placed on the same scale and none of them unduly affects the gradients and weights during flow through the network. For accessing feature importance and interactions, we use the recently open-sourced \textsc{Python} package \texttt{pathexplain}\footnote{\url{https://github.com/suinleelab/path_explain}} \citep{explaining_explanations_hessians}.

% SF: commented to move further
%In addition, we also utilize a robust variational autoencoder (see Section \ref{sec:rvae}) to study the impact of toggling vents between `ON' and `OFF'. The RVAE allows us to isolate out-of-distribution (OOD) samples -- those data points in the training and test sets which are not drawn from the same underlying distribution as the majority of samples in the training set. This serves two purposes. First, it allows us to analyze the impact of vent-toggling only on those samples that are `similar enough' to the majority of samples in the training set, thus increasing our confidence in downstream IQ prediction on these observations. Second, this allows us to suppress the effect of outliers in our measurements. This can be used for anomaly detection and hence predictive maintenance; we relegate this to future work and briefly discuss its implications in Section \ref{sec:conclusion}.

%We also use an off-the-shelf Light GBM model to serve as a baseline against which to measure the performance and validate the effort spent in creating our network. To extract feature importance and interactions from this tree-based model, we use the SHAP package \citep{shap1,shap2}.%; we expound on this in \S\ref{sec:DL_feature_imp}. 

%Fortunately, the past few years have seen extensive research into designing exactly such DNNs, specialized to beat their ML-based cousins on structured data. While some mimic decision tree ensembles \citep{node}, others focus on developing novel architectures using attention \citep{attention_is_all_you_need} suitable for handling tabular data \citep{selfattention_feature_importance, tabnet}. In this work, we use a modified version of the `TabNet' architecture \citep{tabnet}, with several improvements. TabNet uses a sparse, learnable mask on the input features--a kind of soft feature selection that favors the selection of just features that are important for the sample under consideration. It uses a special type of non-linearity called `sparsemax' \textbf{sparsemax citation}, along with an \emph{attention mechanism} \citep{attention_is_all_you_need} called `self-attention' to zero out the contributions of non-relevant features in through a sequence of several steps. TabNet is also able to naturally normalize features of varying ranges, and thus does not require feature pre-processing. For a more detailed description and a visual overview of their network, we refer the readers to \S$2$ and Figure 4, respectively, of \cite{tabnet}. While TabNet has feature interpretability built-in, it can only output the magnitude of the impact of a feature on the output, and not its direction. In other words, it cannot discriminate a feature positively impacting the MPIQ from a feature negatively impacting it, except in magnitude of their effects. For this reason, we do not use this functionality, and instead utilize the \textrm{pathexplain}\footnote{\url{https://github.com/suinleelab/path_explain}} package to obtain feature importance; we expound on this in \S\ref{sec:DL_feature_imp}.\seb{maybe punt some of the description into the related work section? Also: graph NN}.

\iffalse
In short, our inductive bias is that there are (highly) correlated features, so selecting the minimum set of features is the best strategy.

Fortunately, recent developments in attention and sparse regularization now pave the way to learn more efficiently from structured data.
\fi

==> old_related_work.tex <==
\section{Related Work}\label{sec:relatedWork}
\begin{itemize}
    \item def include a couple of plots from racine's work.
\end{itemize}

\iffalse
\begin{figure*}
    %\begin{subfigure}{0.5\textwidth}
    \includegraphics[width=0.9\linewidth]{Cfht Observatory 1-compressed.pdf}
    \label{fig:subim1}
    %\end{subfigure}
    %\begin{subfigure}{0.5\textwidth}
    %\includegraphics[width=0.9\linewidth]{Cfht Observatory 1-compressed.pdf}
    %\label{fig:subim1}
    %\end{subfigure}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{iqcontributions.PNG}
    \caption{https://iopscience.iop.org/article/10.1086/605313/pdf page 919}
    \label{fig:my_label}
\end{figure*}
\fi


\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{tempdelta.PNG}
    \caption{Rene Racine, temperature imbalances in side the dome. https://iopscience.iop.org/article/10.1086/605313/pdf page 909}
    \label{fig:my_label}
\end{figure*}


==> shapley_values.tex <==

\section{Shapley Values}\label{sec:shapley_values} \textbf{COPIED VERBATIM FROM ANOTHER PAPER I AM DRAFTING, WILL BE MODIFIED SUBSTANTIALLY}

Consider a dataset with $N$ features, $X=\left\{X^{(1)}, \ldots, X^{(N)}\right\},$ and a real-valued target variable, $y$. Given an instance (observation) $x \in X,$ a model $v$ forecasts the target as $v[x]$. \emph{Question}--Can we attribute the departure of a prediction $f[x]$ from its average value $\bar{y}$ in terms of the observed instance $x$? In a linear model, the answer is trivial :$v[x]-\bar{y}=\beta_{1} x^{(1)}+\cdots+\beta_{N} x^{(N)}$ (see Fig ()). We would like to do a similar local decomposition for any (non-linear) ML model.\footnote{As explained in \S\ref{} and evident from Figure {}, non-linear models provide much better predictions than linear ones.} Shapley values answer this \emph{attribution} problem through game theory \citep{shapley}. They originated with the purpose of resolving the following scenario--A group of differently skilled participants are all \emph{cooperating} with each other for a collective reward; how should the reward be \emph{fairly} divided amongst the group? In the context of machine learning, the participants are the features of our input dataset input and the collective payout is the model prediction. Here, we use Shapley values to calculate how much each individual feature \emph{marginally} contributes to the model output.

While a goal of this paper is to explain the contribution of each observing band to various galaxy properties, for the sake of simplicity we chose to explain Shapley values using a toy example. Let's say that we operate a small hedge fund, and our team consists of three people: \textbf{A}lice, \textbf{B}ob, and \textbf{C}arol. Everyday they together manage to make \textbf{X = 20} (thousand) dollars. Our year has been very profitable and we would like to distribute a bonus to the team members. In order for us to do that in a fair way we need to find out how much each person contributes to the production of the \textbf{X} dollars.

\begin{enumerate}
    \item First, we consider the $2^{N=3}$ possible coalitions (interactions) between the players (features), where some players (features) may not participate (i.e., remain at their average value), and other may participate (depart from their average value). See Table \ref{table:coalitions}.
    \item Second, we use the coalitions (interactions) table to compute the marginal contribution of each player (feature) conditional to the other players (features). The marginal impact of changing \emph{Alice} after changing \emph{Bob} may differ from the marginal impact of changing \emph{Bob} after changing \emph{Alice}. Accordingly, we must account for all possible $N!$ sequences of conditional effects. See Table \ref{table:marginal_conditional_contribution}.
    \item Finally, the \emph{Shapley value} of a player (feature) is the average conditional marginal contribution of that player across all the possible $N!$ ways of conditioning $v[.]$. See last row of Table \ref{table:marginal_conditional_contribution} and Equation \ref{eq:shapley_main}.
\end{enumerate}

\begin{table*}
\centering
\begin{tabular}{|c|c|c|c|}
\hline $\text{Alice} \neq \overline{\text{Alice}}$ & $\text{Bob} \neq \overline{\text{Bob}}$ & $\text{Carol} \neq \overline{\text{Carol}}$ & $v(...) \left(= v[x \mid \ldots]\right)-\bar{y}$ \\
\hline 0 & 0 & 0 & $v(\varnothing) (= v[x \mid 000])-\bar{y} = 0$ \\
\hline 0 & 0 & 1 & $v(C) (= v[x \mid 001])-\bar{y} = 10$ \\
\hline 0 & 1 & 0 & $v(B) (= v[x \mid 010])-\bar{y} = 5$ \\
\hline 0 & 1 & 1 & $v(B,C) (= v[x \mid 011])-\bar{y} = 7$ \\
\hline 1 & 0 & 0 & $v(A) (= v[x \mid 100])-\bar{y} = 2$ \\
\hline 1 & 0 & 1 & $v(A,C) (= v[x \mid 101])-\bar{y} = 8$ \\
\hline 1 & 1 & 0 & $v(A,B) (= v[x \mid 110])-\bar{y} = 10$ \\
\hline 1 & 1 & 1 & $v(A,B,C) (= v[x \mid 111])-\bar{y} = \textcolor{orange}{20}$ \\
\hline
\end{tabular}
\caption{In a model with 3 features, there are $2^{3}=8$ possible interactions. For each interaction, we compute the departure of the model's forecast from its baseline (average value). We encode as `1' a feature that is not at its average value (it forms part of a \emph{coalition}), and `0' a feature that is at its average value. Thus $v(A,B)=v(B,A)$, $v(B,C)=v(C,A)$, $v(A,C)=v(C,A)$, and $v(A,B,C)=v(B,A,C)=v(A,C,B)$.}
\label{table:coalitions}
\end{table*}

\iffalse
%similar plot to the one in /home/sgilda/Downloads/SSRN-id3637020.pdf, page 9
An attribution of the departure of a model's prediction, $f[x],$ from its average value, $\bar{y}$ Because addition is commutative, the sequence of the effects does not alter the result. Hence,
in a linear model, the attribution is invariant to the sequence of effects.
\fi

%\subsection{Coalitional Game Theory}

\begin{table*}%[h!]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline Combination & \multicolumn{1}{|c|} {Alice} & \multicolumn{1}{|c|} {Bob} & \multicolumn{1}{|c|} {Carol} & Total \\
\hline $\mathrm{A}, \mathrm{B}, \mathrm{C}$ & $v(\mathrm{A})-v(\varnothing) = 2$ & $v(\mathrm{A}, \mathrm{B})-v(\mathrm{A}) = 8$ & $v(\mathrm{A}, \mathrm{B}, \mathrm{C})-v(\mathrm{A}, \mathrm{B}) = 10$ & \textcolor{orange}{20}\\
\hline $\mathrm{A}, \mathrm{C}, \mathrm{B}$ & $v(\mathrm{A})-v(\varnothing) = 2$ & $v(\mathrm{A}, \mathrm{C}, \mathrm{B})-v(\mathrm{A}, \mathrm{C}) = 12$ & $v(\mathrm{A}, \mathrm{C})-v(\mathrm{A}) = 6$ & \textcolor{orange}{20} \\
\hline $\mathrm{B}, \mathrm{A}, \mathrm{C}$ & $v(\mathrm{B}, \mathrm{A})-v(\mathrm{B}) = 5$ & $v(\mathrm{B})-v(\varnothing) = 5$ & $v(\mathrm{B}, \mathrm{A}, \mathrm{C})-v(\mathrm{B}, \mathrm{A}) = 10$ & \textcolor{orange}{20} \\
\hline $\mathrm{B}, \mathrm{C}, \mathrm{A}$ & $v(\mathrm{B}, \mathrm{C}, \mathrm{A})-v(\mathrm{B}, \mathrm{C}) = 13$ & $v(\mathrm{B})-v(\varnothing) = 5$ & $v(\mathrm{B}, \mathrm{C})-v(\mathrm{B}) = 2$ & \textcolor{orange}{20} \\
\hline $\mathrm{C}, \mathrm{A}, \mathrm{B}$ & $v(\mathrm{C}, \mathrm{A})-v(\mathrm{B}) = 3$ & $v(\mathrm{C}, \mathrm{A}, \mathrm{B})-v(\mathrm{C}, \mathrm{A}) = 12$ & $v(\mathrm{C})-v(\varnothing) = 10$ & \textcolor{orange}{20} \\
\hline $\mathrm{C}, \mathrm{B}, \mathrm{A}$ & $v(\mathrm{C}, \mathrm{B}, \mathrm{A})-v(\mathrm{C}, \mathrm{B}) = 13$ & $v(\mathrm{C}, \mathrm{B})-v(\mathrm{C}) = -3$ & $v(\mathrm{C})-v(\varnothing) = 10$ & \textcolor{orange}{20} \\
\hline Average & $6.3$ & $6.5$ & $8$ & \textcolor{orange}{20} \\
\hline
\end{tabular}
\caption{In a model with 3 features, there are $3! = 6$ possible sequences. We can use the interactions table to derive the marginal contribution of each feature in each sequence. The Shapley values are the averages per column.}
\label{table:marginal_conditional_contribution}
\end{table*}

\iffalse
\begin{tabular}{l|l|l|l}
\multicolumn{1}{c|} { Sequence } & \multicolumn{1}{c|} {$x^{(1)}$} & \multicolumn{1}{c} {$x^{(2)}$} & \multicolumn{1}{c} {$x^{(3)}$} \\
\hline$x^{(1)}, x^{(2)}, x^{(3)}$ & $f[x \mid 100]$ & $f[x \mid 110]$ & $f[x \mid 111]$ \\
& $-f[x \mid 000]$ & $-f[x \mid 100]$ & $-f[x \mid 110]$ \\
\hline$x^{(1)}, x^{(3)}, x^{(2)}$ & $f[x \mid 100]$ & $f[x \mid 111]$ & $f[x \mid 101]$ \\
& $-f[x \mid 000]$ & $-f[x \mid 101]$ & $-f[x \mid 100]$ \\
\hline$x^{(2)}, x^{(1)}, x^{(3)}$ & $f[x \mid 110]$ & $f[x \mid 010]$ & $f[x \mid 111]$ \\
& $-f[x \mid 010]$ & $-f[x \mid 000]$ & $-f[x \mid 110]$ \\
\hline$x^{(2)}, x^{(3)}, x^{(1)}$ & $f[x \mid 111]$ & $f[x \mid 010]$ & $f[x \mid 011]$ \\
& $-f[x \mid 011]$ & $-f[x \mid 000]$ & $-f[x \mid 010]$ \\
\hline$x^{(3)}, x^{(1)}, x^{(2)}$ & $f[x \mid 101]$ & $f[x \mid 111]$ & $f[x \mid 001]$ \\
& $-f[x \mid 001]$ & $-f[x \mid 101]$ & $-f[x \mid 000]$ \\
\hline$x^{(3)}, x^{(2)}, x^{(1)}$ & $f[x \mid 111]$ & $f[x \mid 011]$ & $f[x \mid 001]$ \\
& $-f[x \mid 011]$ & $-f[x \mid 001]$ & $-f[x \mid 000]$
\end{tabular}
\fi
%that slide on Interaction Effects. Page 15

\underline{Eliminating Redundancy}: As we can appreciate from the numerical example, some calculations are redundant. For example, the marginal contribution of \emph{(Carol)} on sequence \emph{(Alice, Bob, Carol)} must be the same as the marginal contribution of \emph{(Carol)} on sequence \emph{(Bob, Alice, Carol)} because (a) in both cases \emph{Carol} comes in third position, and (b) the permutations of \emph{(Alice, Bob)} do not alter that marginal contribution. The Shapley value of a feature $i$ can be derived as the average contribution of $i$ across all possible coalitions $S$, where $S$ does not include feature $i$:

\begin{align}\label{eq:shapley_main}
    \phi_{i}(v)=\sum_{S \subseteq N \backslash\{i\}} \frac{|S| !(|N|-|S|-1) !}{|N| !}(v(S \cup\{i\})-v(S))
\end{align}

The above equation describes \emph{coalitional game} (the scenario described previously) with a set \textbf{\emph{N}} of \emph{n} features (players). The function $v$ gives the value (payout) for any subset of those features (players). For example, if $S$ be a subset of \textbf{\emph{N}}, then \emph{v(S)} gives us the value of that subset. Thus for a coalitional game \emph{(N, v)} Equation \ref{eq:shapley_main} outputs the value for feature \emph{i}, i.e. its the Shapley value.\footnote{Equation \ref{eq:shapley_main} computes the exact Shapley values by grouping the marginal conditional contributions in terms of coalitions $(S)$. For large $N,$ \cite{shap1} and \cite{shap2} have developed fast algorithms for the estimation of $\phi_{i}$} For ease of explanation, we focus our attention on calculating how many of the $X$ dollars can be attributed to \textbf{C}(arol), i.e. calculating the Shapley value for \textbf{C}. We then examine the various components of Equation \ref{eq:shapley_main} and study their significance.
\begin{itemize}
    \item If we relate this back to the parameters of the Shapley value formula we have $N = \{A, B, C\}$ and $i = C$. The highlighted section in Equation \ref{eq:shapley_highlight_0} (derived from Equation \ref{eq:shapley_main} by re-arranging some terms) says that we need to take our group of people and exclude the person that we are focusing on now. Then, we need to consider all of the possible subsets that can be formed. So if we exclude \textbf{C} from the group we are left with \emph{{A, B}}. From this remaining group we can form the following subsets (i.e. these are the sets that \emph{S} can take on): $\varnothing, A, B, AB$. In total, we can construct four unique subsets from the remaining team members, including the null set.
    \begin{align}\label{eq:shapley_highlight_0}
    \phi_{i}(v)=\frac{1}{|N|} \sum_{\textcolor{orange}{S \subseteq N \backslash\{i\}}}\left(\begin{array}{c}
    |N|-1 \\
    |S|
    \end{array}\right)^{-1}(v(S \cup\{i\})-v(S))
    \end{align}
    \item Next, we focus on the highlighted term  in Equation \ref{eq:shapley_highlight_1}.
    \begin{align}\label{eq:shapley_highlight_1}
    \phi_{i}(v)=\frac{1}{|N|} \sum_{S \subseteq N \backslash\{i\}}\left(\begin{array}{c}
    |N|-1 \\
    |S|
    \end{array}\right)^{-1}\textcolor{orange}{(v(S \cup\{i\})-v(S))}
    \end{align}
    This refers to the \emph{marginal value} of adding feature (player) $i$ to the dataset (game). Specifically, we want to see what the difference in the money earned daily if we add $C$ to each of our 4 subsets. We can represent these 4 marginal values visually as: $\Delta v_{C, \varnothing}, \Delta v_{AC, A}, \Delta v_{BC, B}, \Delta v_{A B C, A B}$. Each of these as a different scenario that we need to observe in order to fairly assess how much \textbf{C} contributes to the overall profit. This means that we need to observe how much money is produced if no one is working (i.e. the empty set $\varnothing$) and compare it to what happens if we only have \textbf{C} working. We also need to observe how much profit is earned by \textbf{A} and \textbf{B} working simultaneously and compare that to the profit earned by \textbf{A} and \textbf{B} together with \textbf{C}, and so on.
    \item Next, the summation in the Shapley value equation is telling us that we need to add all them together. However, we also need to scale each marginal value before we do that, which we are provided this prescription by the highlighted part in Equation \ref{eq:shapley_highlight_2}.
    \begin{align}\label{eq:shapley_highlight_2}
    \phi_{i}(v)=\frac{1}{|N|} \sum_{S \subseteq N \backslash\{i\}}\textcolor{orange}{\left(\begin{array}{c}
    |N|-1 \\
    |S|
    \end{array}\right)^{-1}}(v(S \cup\{i\})-v(S))
    \end{align}
    It calculates how many permutations of each subset \emph{size} we can have when constructing it out of all remaining team members excluding feature (player) \emph{i}. In other words, given \textbf{$\lvert$N$\rvert$-1} features (players), how many groups of size \textbf{$\lvert$S$\rvert$} can one form with them? We then use this number to divide the marginal contribution of feature (player) $i$ to all groups of size \textbf{$\lvert$S$\rvert$}. For our scenario, we have that \textbf{$\lvert$N$\rvert$-1 = 2}, i.e. these are the remaining team members when we are left with when calculating the Shapley value for \textbf{C}. In our case we will use that part of the equation to calculate how many groups we can form of size 0, 1, and 2, since those are only group sizes we can construct with the remaining players. So, for example, if we have that \textbf{$\lvert$S$\rvert$ = 1} then we get that we can construct 2 different groups of this size: \emph{A} and \emph{B}. This means that we should apply the following scaling factors to each of our 4 marginal values: $1\Delta v_{C, \varnothing}, \frac{1}{2}\Delta v_{A C, A}, \frac{1}{2}\Delta v_{B C, B}, 1\Delta v_{A B C, A B}$. By adding this scaling factor we are \emph{averaging out} the effect that the rest of the team members have for each subset size. This means that we are able to capture the \emph{average} marginal contribution of \textbf{C} when added to a team of size 0, 1, and 2 \emph{regardless} of the composition of these teams.
    \item Next, we focus on the remaining term, highlighted in Equation \ref{eq:shapley_highlight_3}.
    \begin{align}\label{eq:shapley_highlight_3}
    \phi_{i}(v)=\textcolor{orange}{\frac{1}{|N|}} \sum_{S \subseteq N \backslash\{i\}}\left(\begin{array}{c}
    |N|-1 \\
    |S|
    \end{array}\right)^{-1}(v(S \cup\{i\})-v(S))
    \end{align}
    So far we have averaged out the effects of the other team members for each subset size, allowing us to express how much \textbf{C} contributes to groups of size 0, 1, and 2. The final piece of the puzzle is to \emph{average out} the effect of the group size as well, i.e. how much does \textbf{C} contribute \emph{regardless} of the size of the team (number of explanatory features in the data set). For our scenario we do this by dividing with 3 since that is the number of different group sizes that we can consider. With this final step, we arrive at the point where can finally compute the Shapley value for \textbf{C}. We have observed how much she marginally contributes to all different coalitions the team that can be formed. We have also averaged out the effects of both team member composition as well as team size which finally allows us to compute the Shapley value for \textbf{C}:
    \begin{align}\label{eq:shapley_final}
        \phi_{C}(v) &= \frac{1}{3} \sum\left(1\Delta v_{C, \varnothing}, \frac{1}{2} \Delta v_{A C, A}, \frac{1}{2} \Delta v_{B C, B}, 1\Delta v_{ABC, AB}\right) \nonumber \\
        &= \frac{1}{3} \sum\left(1\times 10, \frac{1}{2} \times 6, \frac{1}{2} \times 2, 1\times 10\right) \nonumber \\
        &= 8
    \end{align}
    Comparing Equation \ref{eq:shapley_final} with the Shapley value for \textbf{C} in the last row of Table \ref{table:marginal_conditional_contribution}, we see that they match exactly.
\end{itemize}

After we have calculated the Shapley values for the rest of the features (players), we will know their individual contributions to the \textbf{X} dollars earned daily, allowing us to fairly divide the year-end bonus amongst all team members:
\begin{align}
    X &=v(\{A, B, C\}) \nonumber \\
    &=\phi_{A}(v)+\phi_{B}(v)+\phi_{C}(v)
\end{align}
This is also evident from the last row of Table \ref{table:marginal_conditional_contribution}, where the Shapley values for \textbf{A}, \textbf{B}, and \textbf{C} add to the total of 20.


\underline{Interaction Effects}: An interaction effect occurs when the effect of one variable on the output depends on the value of another variable. The estimation of interaction effects requires having an accurate attribution of the individual effect of the variables involved. This makes Shapley values particularly useful for estimating these. For $i \neq j$:
\begin{align}
    \phi_{i, j}=\sum_{S \subseteq(X \backslash\{i, j\})} \frac{\|S\| !(N-\|S\|-2) !}{2(N-1) !} \delta_{i, j}[S], \nonumber \\
    \delta_{i, j}[S]=v[S \cup\{i, j\}]-v[S \cup\{i\}]-v[S \cup\{j\}]+f[S]
\end{align}

\underline{Properties}:
This method is the provably [citation required] the only one that satisfies four axioms of \emph{fair} credit-attribution:
\begin{enumerate}
    \item \emph{Efficiency}: The sum of the Shapley values of all features (players) equals the value of the total coalition. That is, the value of $X = 20$ in the bottom-rightmost corner in Table \ref{table:coalitions} is the same as the $20$ in the bottom-rightmost cell in Table \ref{table:marginal_conditional_contribution}.
    \item \emph{Dummy Player}: If a feature (player) never adds any marginal value regardless of the coalition, its payoff (Shapley value $\phi_{i}(v)$) is 0.
    \item \emph{Symmetry}: All players have a fair chance to join the game. That’s why Table \ref{table:coalitions} lists all the permutations of the players. If two players always add the same marginal value to any subset to which they are added, their payoff portion should be the same. In other words, $\phi_{i} = \phi_{j}$ IIF feature \emph{i} and feature \emph{j} contribute equally to all possible coalitions.
    \item \emph{Additivity}: A function with combined outputs has as Shapley values the sum of the constituent ones. For any pair of games $v, w$, $\phi(v+w) = \phi(v)+\phi(w)$, where $(v+w)(S)=v(S)+w(S) \forall S$. This property allows us to combine Shapley values from $n$ different models, thus enabling interpretability for ensembles. 
\end{enumerate}



==> ssl.tex <==
\subsection{Semi-Supervised Learning}\label{sec:DL_SSL}
Semi-supervised learning (SSL) is a domain of machine learning which allows us to combine (typically a small amount) of labeled data with (typically a larger amount) of unlabeled data during training. SSL falls somewhere between unsupervised learning--with no labeled training data--and supervised learning--with only labeled training data. The primary goal while employing an SSL framework is to use the unlabeled dataset to guide our model's predictions on the labeled dataset. A secondary goal shared by some methods--including the one we employ in this work--is to label the unlabeled data using the labeled information set.

While there exists a plethora of methods, both simple and complex, in this domain, and the development of SSL algorithms to solve problems in real-time is an area of active research \textbf{CITATION NEEDED}, we use an algorithm of the type that solves SSL by generating pseudo-labels for the unlabelled data. `Speed as a Supervisor' (SaaS, \cite{saas1}) enables us to generate pseudo-labels concurrently with estimating the parameters of our deep learning model. Ussing SaaS we are able to obtain (potentially accurate) estimates for the unlabeled data at the end of training. \cite{saas1} empirically show that corollary to widely known fact that accurate labels lead to fast training \citep{good_labels_leadsto_fast_training}, fast training is also a good indicator of good labels. Specifically, the algorithm consists of two loops: in the inner loop, SaaS aims to find a set of pseudo-labels that decreases the loss function over a small number of epochs, the most; in the outer loop, we optimize ofer the posterior distribution of the pseudo labels \cite{saas2} \yst{what is being optimized here? Is it the similarity between the label distribution of the labelled training set vs. the pseudo labels? If so, why is that a good assumption?}. We show this process via a cartoon in Figure()(), where we use our modified TabNet in the inner loop.

%figure and algo, consider https://openaccess.thecvf.com/content_CVPR_2020/papers/Lokhande_Generating_Accurate_Pseudo-Labels_in_Semi-Supervised_Learning_and_Avoiding_Overconfident_Predictions_CVPR_2020_paper.pdf


==> tabnet.tex <==
\subsection{Deep Learning for Tabular Data}\label{sec:DL_tabnet}
Given the ease of use and conventionally superior performance of tree-based models on tabular data, it is natural to ask--why consider DNNs at all?
\begin{itemize}
    \item DNNs are powerful feature pre-processors. Using back-propagation, they learn a fine-tuned heirarchical representation of data by mapping input features to the output label(s). This allows us to shift our focus from feature engineering to fine-tuning the architecture, designing better loss functions, and generally experimenting with the mechanics of our neural network. This exactly functionality allows us to get away with merely using the pairwise differences of the temperature values in \S\ref{sec:data_cleaning_feature_engineering} as additional, hand-crafted features.
    \item There is empirical proof that DNNs result in improved performance with larger sized datasets \citep{airbnb}.
    \item Deep learning allows us to train systems end-to-end, which unlocks the possibility of using unlabelled samples to better predict the labelled ones (\emph{semi-supervised learning}, \S\ref{sec:DL_SSL}).
    \item It is easier to use DNNs in an online-mode, with data points `streaming in' rather than arriving in batches. This is because tree-based models need access to all the data to determine best split points, and hence need to be trained every time a new observation comes in. While this work does not use streaming data, in preparation for our future work on real-time predictions we believe it best to move to a neural network from the get-go.
\end{itemize}

==> to_do.tex <==

\section{To Do}\label{sec:to_do}
\begin{itemize}
    \item Better abstract
    \item More comprehensive introduction
    \item Transfer material from Rene Recine's old report to `Related Work' section
    \item Come up with a cool name for the deep-net; helpful phrases: `tabnet', `stacked', `mixture density network', `imputation', `modified', `seeing', `image quality'.
    \item in `related work', make sure to end with what results we should expect from the deep net. this will be a `quasi-ground truth' agaist which to compare results.
    \item in `results' (`discussion'?), compare insights obtained from DL with those expected from above. highlight gains.
    \item make a list of limitations, both from ML perspective and science/seeing perspective
    \item talk to CFHT folks about `future work'.
    \begin{itemize}
        \item end to end pipeline incorporating imputation
        \item higher resolution in vent configuration
        \item explore pairwise feature interaction like in \cite{shap1, shap2}.
        \item propagation of observational errors
        \item feature importance based on errors as opposed to median outputs
    \end{itemize}
    \item Ask Andy to populate `Acknowledgements'
    \item WHAT IF plots: what happens when we change vent configurations?
    \item check with Andy about public vs private nature of data
    \item Include in Appendix analysis highlighting the importance of having probabilistic predictions per data point. Cf. discussion with YST on 07-10-2020.
\end{itemize}

